RL-MUL 2.0: Multiplier Design Optimization with Parallel Deep Reinforcement Learning and Space Reduction

Multiplication is a fundamental operation in many applications, and multipliers are widely adopted in various circuits. However, optimizing multipliers is challenging due to the extensive design space. In this paper, we propose a multiplier design optimization framework based on reinforcement learning. We utilize matrix and tensor representations for the compressor tree of a multiplier, enabling seamless integration of convolutional neural networks as the agent network. The agent optimizes the multiplier structure using a Pareto-driven reward customized to balance area and delay. Furthermore, we enhance the original framework with parallel reinforcement learning and design space pruning techniques and extend its capability to optimize fused multiply-accumulate (MAC) designs. Experiments conducted on different bit widths of multipliers demonstrate that multipliers produced by our approach outperform all baseline designs in terms of area, power, and delay. The performance gain is further validated by comparing the area, power, and delay of processing element arrays using multipliers from our approach and baseline approaches.

==> doc/answer.tex <==
\begin{@twocolumnfalse}
%\onecolumn
%\normalsize

\noindent\textbf{Responses to reviewers and editor}



\section*{\textbf{Reviewer 2}}

\begin{myblock}{Comment 2-1}
The authors has addressed all the reviewer's suggestion, but one thing is missing.

The author's  main motto  along with  “Deep Reinforcement Learning” is a merged MAC.
Whatever was asked last time to refer to the paper  is not to just cite  in the paper, but that paper also has the same  “merged MAC” approach and how the author's approach is different / better than it.
“Mohamed Asan Basiri M and Noor Mahammad Sk. 2014. An Efficient Hardware-Based Higher Radix Floating Point MAC Design. ACM Trans. Des. Autom. Electron. Syst. 20, 1, Article 15 (November 2014), 25 pages. https://doi.org/10.1145/2667224”

\end{myblock}
\textbf{Author's answer:}
Thank you for your comments. 
In our revised manuscript, we will clarify the similarities and differences between our RL-MUL and the merged MAC in the TODAES’14 paper. 
While both share the basic idea of using the result of the previous MAC operation as a partial product to reduce delay and area, the key differences are as follows:

\textit{Application Domain:}
TODAES’14 focuses on floating-point MAC designs, incorporating additional operations like exponent alignment, rounding, and normalization to handle IEEE-754 floating-point arithmetic. 
RL-MUL targets integer binary MAC designs, avoiding the complexity of floating-point-specific operations for a more efficient hardware implementation.

\textit{Encoding Method:}
TODAES’14 uses high-radix Booth encoding (e.g., radix-4, radix-8, radix-16) to reduce the number of partial products. 
RL-MUL employs both AND-based encoding and Booth Radix-4 encoding, dynamically optimized using reinforcement learning to suit specific objectives.

\textit{Compression Tree:}
TODAES’14 uses fixed Wallace and Braun trees for partial product reduction. 
RL-MUL leverages reinforcement learning to explore and optimize the compression tree structure, achieving better PPA (performance, power, area) metrics.

\textit{Contribution Focus:}
TODAES’14’s primary contribution lies in proposing a novel floating-point MAC structure, which optimizes performance and area by introducing techniques such as high-radix Booth encoding, tailored exponent alignment, and efficient normalization processes. 
This design specifically addresses the challenges of floating-point arithmetic under IEEE-754 standards.

In contrast, our primary contribution is the development of RL-MUL, a reinforcement learning-based framework for automating the optimization of multiplier compression tree structures.
In RL-MUL 2.0, we extend this optimization framework to Merged MAC designs. 
By leveraging the Merged MAC structure, we enable the methodologies and optimization strategies developed for multipliers to be applied to MAC designs. 

It is important to note that our contribution does not lie in the innovation of the MAC structure itself but in the application of reinforcement learning to automate and enhance the optimization process.
    
\textbf{Author's action:}
In \Cref{sec:intro}, we have added a detailed description of the Merged MAC design in the TODAES'14 paper.



\end{@twocolumnfalse}

==> doc/cover.tex <==
{
%\twocolumn[
%\begin{@twocolumnfalse}
%\large

\noindent Dear Editor and Reviewers,

\ \\
Thank you very much for reviewing and editing our submission.
A preliminary version of this work was presented at the 2023 ACM/IEEE Design Automation Conference (DAC).
This journal version is extended to include enhancements, analysis, and additional experiments not presented in the conference paper.


\ \\
The main differences between this revised submission and previous version are listed below:

\begin{enumerate}
    \item{
    In \Cref{sec:intro}, we have added a detailed description of the Merged MAC design in the TODAES'14 paper.
    }
        \item{
       We have provided a detailed response to reviewer comment, along with corresponding action, which are included at the end of the manuscript.
    }

    
\end{enumerate}

\ \\
Your time and effort spent in reviewing this paper would be greatly appreciated.

\ \\
Best regards,

\ \\

\noindent 
Dongsheng Zuo, Jiadong Zhu, Yikang Ouyang, Yuzhe Ma

%\end{@twocolumnfalse}
%]
}
